A One-Size-Fits-All Approach to Improving Randomness in Paper Assignment

The assignment of papers to reviewers is a crucial part of the peer review processes of large publication venues, where organizers (e.g., conference program chairs) rely on algorithms to perform automated paper assignment. As such, a major challenge for the organizers of these processes is to specify paper assignment algorithms that find appropriate assignments with respect to various desiderata. Although the main objective when choosing a good paper assignment is to maximize the expertise of each reviewer for their assigned papers, several other considerations make introducing randomization into the paper assignment desirable: robustness to malicious behavior, the ability to evaluate alternative paper assignments, reviewer diversity, and reviewer anonymity. However, it is unclear in what way one should randomize the paper assignment in order to best satisfy all of these considerations simultaneously. In this work, we present a practical, one-size-fits-all method for randomized paper assignment intended to perform well across different motivations for randomness. We show theoretically and experimentally that our method outperforms currently-deployed methods for randomized paper assignment on several intuitive randomness metrics, demonstrating that the randomized assignments produced by our method are general-purpose.

==> preliminaries.tex <==
We consider the standard conference peer review setting in which a set $\P$ of $\np$ papers need to be assigned to a set $\R$ of $\nr$ reviewers. Each paper $p$ in $\P$ should be assigned to $\lp$ reviewers and each reviewer $r$ in $\R$ should receive no more than $\lr$ papers. In this work, we consider both deterministic and randomized assignments. A deterministic assignment is represented as a matrix $\x$ in $\{0,1\}^{\np\times \nr}$, where $x_{p,r} =1 $ indicates that paper $p$ is assigned to reviewer $r$. Similarly, a randomized assignment is represented as a matrix $\x$ in $[0,1]^{\np\times \nr}$, where $x_{p, r}$ denotes the marginal probability that paper $p$ is assigned to reviewer $r$. For both deterministic and randomized assignments, $\x$ is feasible if each of its rows sums to $\lp$ and each of its columns sums $\leq \lr$. It has been shown in previous works \cite{budish2009implementing, jecmen2020mitigating} that a feasible randomized assignment $\x$ can always be implemented as a distribution of feasible deterministic assignments, and \cite{jecmen2020mitigating} provides an efficient procedure for sampling a deterministic assignment from a given randomized assignment. In this work, we consider only the problem of computing randomized assignments; in practice, the procedure of \cite{jecmen2020mitigating} can be used for sampling. %We thereby consider randomized assignments in the scope of this paper. 

As commonly studied in previous works, we assume that a similarity matrix $\S$ in $\mathbb R_{\geq 0}^{\np\times \nr}$ is given. Here, $S_{p,r}$ represents the predicted quality of review from reviewer $r$ for paper $p$ and is generally computed from various sources~\cite{shah2022challenges}: reviewer and paper subject areas, reviewer-selected bids, and textual similarity between the paper and the reviewer's past work~\cite{mimno07topicbased, liu14graphpropagation, rodriguez08coauthorsip, tran17expertsuggestion, charlin13tpms}. The \textbf{quality} of an assignment is defined as the (expected) total similarity of all assigned paper reviewer pairs, i.e., 
$
    \quality(\x)=\sum_{p,r}x_{p,r}S_{p,r}. 
$
One standard approach for computing a paper assignment is to maximize quality~\cite{charlin13tpms, Long13gooadandfair, goldsmith07aiconf, tang10constraied, flach2010kdd, taylor08assignment, Charlin2011AFF}, resulting in a deterministic assignment. Variants of this approach have been widely used by existing conferences, such as NeurIPS, AAAI, and ICML~\cite{shah2022challenges}. 


While the deterministic maximum-quality assignment is the most common, there are various reasons why randomized paper assignment may be beneficial. Previous work~\cite{jecmen2020mitigating} has proposed an algorithm for computing randomized paper assignments: \textbf{Probability Limited Randomized Assignment (PLRA)}. For a given parameter $Q\in [0,1]$, solve:
\begin{equation*}
	\begin{array}{lll}
		\textup{Maximize} & \quality(\x) \\
		\textup{Subject to} & \sum_r x_{p,r}=\lp &\forall p\in\P,\\
		& \sum_p x_{p,r}\leq \lr &\forall r\in\R,\\
		& 0\leq x_{p,r}\leq Q & \forall p\in\P,r\in\R.
	\end{array}\tag{PLRA}
\end{equation*}
The solution $\x$ to this program will be a randomized assignment. %By limiting each entry of $\x$ to be at most $Q$, PLRA guarantees that any malicious reviewer aiming to be assigned to a target paper has at most probability $Q$ to succeed, even if the reviewer and paper are chosen adversarially. 
The hyperparameter $Q$ can be adjusted to balance the loss in quality and level of randomization. PLRA has been deployed in iterations of the AAAI conference~\cite{shah2022challenges} and is implemented at the popular conference management system OpenReview.net~\cite{openreviewmatcher}. For the rest of the paper, we consider PLRA as a benchmark algorithm for randomized paper assignment. We note that in the original formulation of~\cite{jecmen2020mitigating}, the value of $Q$ could be set to different values for each pair $(p, r)$. However, this level of flexibility makes it a significant challenge for program chairs to choose appropriate hyperparameters, and as a result only the single-hyperparameter version stated in PLRA has been deployed in practice. 
